High-Speed Resource Allocation Algorithm Using a Coherent Ising Machine for NOMA Systems

Non-orthogonal multiple access (NOMA) technique is important for achieving a high data rate in next-generation wireless communications. A key challenge to fully utilizing the effectiveness of the NOMA technique is the optimization of the resource allocation (RA), e.g., channel and power. However, this RA optimization problem is NP-hard, and obtaining a good approximation of a solution with a low computational complexity algorithm is not easy. To overcome this problem, we propose the coherent Ising machine (CIM) based optimization method for channel allocation in NOMA systems. The CIM is an Ising system that can deliver fair approximate solutions to combinatorial optimization problems at high speed (millisecond order) by operating optimization algorithms based on mutually connected photonic neural networks. The performance of our proposed method was evaluated using a simulation model of the CIM. We compared the performance of our proposed method to simulated annealing, a conventional-NOMA pairing scheme, deep Q learning based scheme, and an exhaustive search scheme. Simulation results indicate that our proposed method is superior in terms of speed and the attained optimal solutions.

==> name.tex <==
\section{Introduction}
\label{sect:introduction}

With the rapid increase in the number of mobile devices, there is an urgent need to increase the spectrum efficiency of mobile communications\cite{1}. 
%Recently, the standardization of the fifth generation communication (5G) is commenced, and 
A non-orthogonal multiple access (NOMA) technique has been proposed as one of the candidate technologies to meet the requirements of the next generation of wireless networks \cite{2,3}. 
Unlike conventional orthogonal multiple access (OMA) schemes, NOMA schemes can effectively increase the spectrum efficiency by introducing extra-power-domains, which enables the data of multiple different users to be multiplexed on the same channel \cite{3}.
More specifically, by applying superposition coding in the transmitter and successive interference cancellation (SIC) technology in the receiver, signals from multiple users that are multiplexed can be distinguished.

In a NOMA system, resources such as channels and power must be appropriately allocated to improve the system performance, such as the data rate, and avoid system outages such as an SIC error \cite{4,21a}.
%Therefore, for a practical NOMA system, it is necessary to formulate joint channel and power allocation problems and obtain an optimal solution.
Previous studies have shown that optimal resource allocation (RA) can increase the total achievable data rate of a system in comparison with random RA \cite{5}. 
Specifically, channel allocation methods that consider the differences in channel gain between users, and power allocation methods that balance system data rates and user fairness, are key aspects in a NOMA system design.
In addition, it is important to allocate resources to avoid the failure conditions of SIC and maximize the performance, including the total data rate, quality of service (QoS), or fairness of the NOMA system. However, joint channel and power allocation problems have been proven to be NP-hard \cite{6}, and their high complexity hinders an efficient and reliable RA, resulting in a low performance of NOMA systems.

To solve the NP-hard RA optimization  problems in NOMA systems, many approaches such as machine learning (ML) and heuristic approaches have been proposed  \cite{7,20,21,17,18,19,21a}.
Optimization using ML has the advantage of a rapid RA in large-scale problems by using trained models that have been learned in advance. However, a trained model may no longer be usable and must be retrained when the system environment changes. 
This has a disadvantage that the RA may not be sufficiently fast when the communication environments change.
By contrast, optimization using heuristic methods is faster owing to a lower computational complexity; however, a fundamental trade-off emerges between the solution accuracy and computational complexity.
By contrast, hardware-based search algorithms, such as quantum computers and Ising machines, have been proposed and are expected to solve various optimization problems at high speeds\cite{9,10,11,12,12a}.
As described in \cite{34}, quantum technologies are emerging technologies that are expected to be deployed in 6G networks around 2030, although it is still unclear when a practical quantum computer will be available.
D-wave\cite{9} is a quantum annealing machine that has already been commercialized and is available for general users. The coherent Ising machine (CIM) \cite{10,11,12,12a} is an  optimization machine based on laser networks, which can deliver fair approximate solutions to combinatorial optimization problems at high speed on the order of milliseconds.
Many NP-complete and NP-hard problems can be  transformed into ground-state search problems of the Ising model \cite{13a}.
Here, the CIM and D-Wave are Ising machines that can rapidly obtain a state near the ground state of the Ising Hamiltonian which represents a good solution to the optimization problem.
As the main difference between the D-Wave and CIM, D-Wave reproduces a coupling of magnetic spins with a chimera topology having sparse connections, whereas in CIM, the Ising network of optical pulses generated by a laser oscillator is fully coupled\cite{10,11}. 

A previous study \cite{12} demonstrated that the CIM is more effective than D-Wave for large-scale large-density problems, and it will be more suitable for the next-generation large-scale wireless communications. In \cite{12a}, the authors showed that 100,000 fully connected spins can be implemented using the CIM. In previous studies \cite{13,14,24,25}, various wireless communication systems are optimized using CIMs. A CIM-based optimization approach has been applied to solve the NP-hard optimization problems in wireless communications. In \cite{16}, it is shown that the optimal solutions obtained can be empirically scaled as $O(1)$ using the CIM. It is therefore possible to achieve a real-time optimization of RA in a large-scale NOMA system using the CIM. In this paper, we propose a RA method for NOMA systems using the CIM. The main contributions of this paper can be summarized as follows.

\begin{itemize}
\item We propose a high-speed RA method using a CIM for NOMA systems, especially for the channel assignment. The proposed method is a hardware-based method with superior speed (milliseconds-order) compared to other existing methods.
\item To the best of our knowledge, previous works related to RA using the CIM in wireless communication assumed that only one user could access each channel simultaneously. In contrast to previous studies, this study focuses on the RA optimization problem using the CIM for NOMA systems where multiple users can be multiplexed in the same channel. Hence, novel solutions are necessary to solve such problems which are different from those in our previous work. For instance, dummy users need to be introduced and the constraints are different, which leads to different strength of the interaction between spins and that of the external magnetic field on each spin. In this study, we formulated the RA combinatorial optimization problem carefully to meet the characteristics of the RA in the NOMA system and the feasibility of solving it using the CIM.
\item To solve the RA optimization problem in NOMA systems using the CIM, it is necessary to derive the parameters of the Ising model and introduce them into the CIM. Therefore, we first transformed the formulated RA combinational problem into a ground state search problem of the Ising Hamiltonian. Then, we derived the parameters of the Ising model that needed to be introduced into the CIM to obtain the solutions, i.e., the interaction between spins and the external magnetic field.
\item To verify the effectiveness of the proposed method, we first evaluated the convergence of the proposed method. Simulation results demonstrated the convergence of the proposed methods. Then, we evaluated the performance of the proposed method in the total data rate and compared it with that of other methods including simulated annealing (SA), exhaustive search (ES), the conventional-NOMA (C-NOMA), and random methods. The simulation results indicate that our proposed approach can achieve higher data rates than other methods. Moreover, the computation time of the proposed, SA, and ES methods was evaluated, which demonstrates that the proposed method can obtain better performance at faster speed.
\end{itemize}

The rest of this paper is organized as follows. Section \Rmnum{2} reviews previous related studies. Section \Rmnum{3} introduces the system model and problem formulation. Section \Rmnum{4} introduces the principle of the CIM in solving the optimization problems.
Section \Rmnum{5} presents the proposed CIM-based RA method for NOMA systems.
Section \Rmnum{6} demonstrates the simulation results.
Section \Rmnum{7} describes future work.
Section \Rmnum{8} provides some concluding remarks regarding this research. 
